SPECWANDS: An Efficient Priority-based Scheduler Against Speculation Contention Attacks

Transient Execution Attacks (TEAs) have gradually become a major security threat to modern high-performance processors. They exploit the vulnerability of speculative execution to illegally access private data, and transmit them through timing-based covert channels. While new vulnerabilities are discovered continuously, the covert channels can be categorised to two types: 1) Persistent Type, in which covert channels are based on the layout changes of buffering, e.g. through caches or TLBs; 2) Volatile Type, in which covert channels are based on the contention of sharing resources, e.g. through execution units or issuing ports. The defenses against the persistent-type covert channels have been well addressed, while those for the volatile-type are still rather inadequate. Existing mitigation schemes for the volatile type such as Speculative Compression and Time-Division-Multiplexing will introduce significant overhead due to the need to stall the pipeline or to disallow resource sharing. In this paper, we look into such attacks and defenses with a new perspective, and propose a scheduling-based mitigation scheme, called SPECWANDS. It consists of three priority-based scheduling policies to prevent an attacker from transmitting the secret in different contention situations. SPECWANDS not only can defend against both inter-thread and intra-thread based attacks, but also can keep most of the performance benefit from speculative execution and resource-sharing. We evaluate its runtime overhead on SPEC 2017 benchmarks and realistic programs. The experimental results show that SPECWANDS has a significant performance advantage over the other two representative schemes.

==> 12-ack.tex <==
%\vspace{-1em}
\ifCLASSOPTIONcompsoc
  % The Computer Society usually uses the plural form
  \section*{Acknowledgments}\label{sec:ack}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}\label{sec:ack}
\fi
This research was supported by the National Natural Science Foundation of China (NSFC) under grant 61902374 and U1736208, and Innovation Funding of ICT, CAS under grant No.E161040. %Pen-Chung Yew is supported by the NSF under the grant CNS-1514444.
The statements in the paper are solely the responsibility of the authors.

==> 5-problem.tex <==
\section{Overview}\label{sec:overview}
In this paper, we attempt to efficiently defeat against all Speculation Contention Attacks (SCAs), including inter-thread and intra-thread mode. 
%Our motivation is to allow most operations can occupy their resource quickly and safely. 
First, we revisit the handicap of existing two defense approaches. For "Time-Division Multiplexing", inflexible time slice partition scheme cannot suffice the demand of various workloads. For "Speculative Compression", when branch occurs frequently and the resolving time is quite long (nearly average 20 cycles for SPEC benchmarks according to our evaluation), the aggregation cost of issuing delay will introduce a huge performance overhead. 
Considering a normal situation as \autoref{fig:example} shows, two HTs execute the same loop snippet. In each iteration, the division operation within the loop body need to be delayed until the guarding branch is resolved, i.e. the operation become non-speculative). As the loop iterates more than 10 times, the overhead can even reaching 20X. 

\bheading{Our Insight.} The observation motivates us to think that \emph{if the scheduler batch multiple speculative operations from same HT into a group so that them can exclusive occupy the resource for a period, then it can compressed the delay between each group members.} However, making such grouping secure for both inter-/intra-thread modes must overcome the following two challenges: 1) how to divide a group within the HT and switch the groups across multiple HTs to avert group interference be exploited by inter-thread attackers; 2) how to eliminate rewinding competition among speculative operations within each group to against intra-thread attackers.

% %No matter how TEAs evolve,
% The root cause of TEAs can be summarized to the violation of \emph{Speculative Non-interference (SNI)} principle\cite{?}. It allows an attacker to leak the system information via the side effects incurred during a speculative execution. As for SCAs, the subset of TEAs that leverages contention-based covert channels, we further conclude the following two critical requirements.

% \begin{mdframed}
% \bheading{Speculative Dependence.} The contention created at the shared component by the sender must explicitly or implicitly depends on the secret value obtained by the accessor during a speculation period.

% \bheading{Unrestricted Access Control.} The shared component must have a \emph{fair-access} policy, e.g. First-Coming-First-Service (FCFS), to all requests, which allows the sender to launch a burst of requests to monopolize its occupancy. 
% \end{mdframed}

% As described in \autoref{subsec:mitigations}, \emph{Speculation Compression} approaches try to cut off the source of speculative dependence, while \emph{Time-Division-Multiplexing} approaches try to break the fair-access policy by partitioning the resource for each thread. However, those approaches all inevitably incur substantial performance overheads.

% \bheading{Our Insight.} 
% We argue that, for different contention situations, we can adopt different \emph{priority-based scheduling policies} to break either one of the two requirements mentioned more intelligently. From the \emph{Speculative Dependence} requirement, we observe that \emph{the sender needs to be speculative throughout the time period of contention, and such speculation will eventually be squashed. While the receiver can be either speculative or non-speculative during this period.} Therefore, the scheduler can assign a higher priority to non-speculative requestor to ensure that no delay happens if it is the receiver. \tbw{This principle can breach the \emph{???} requirement}. When all requestors are speculative, the scheduler can set the priority according to other speculation-independent factors, to ensure the delay of a speculative receiver is not caused by the sender. 
